Optimal multi-action treatment allocation: A two-phase field experiment to boost immigrant naturalization

Research underscores the role of naturalization in enhancing immigrants' socio-economic integration, yet application rates remain low. We estimate a policy rule for a letter-based information campaign encouraging newly eligible immigrants in Zurich, Switzerland, to naturalize. The policy rule assigns one out of three treatment letters to each individual, based on their observed characteristics. We field the policy rule to one-half of 1,717 immigrants, while sending random treatment letters to the other half. Despite only moderate treatment effect heterogeneity, the policy tree yields a larger, albeit insignificant, increase in application rates compared to assigning the same letter to everyone.

==> partialinput.tex <==
\makeatletter
\newread\pin@file
\newcounter{pinlineno}
\newcommand\pin@accu{}
\newcommand\pin@ext{pintmp}
% inputs #3, selecting only lines #1 to #2 (inclusive)
\newcommand*\partialinput [3] {%
\IfFileExists{#3}{%
\openin\pin@file #3%
% skip lines 1 to #1 (exclusive)
\setcounter{pinlineno}{1}%
\@whilenum\value{pinlineno}<#1 \do{%
\read\pin@file to\pin@line%
\stepcounter{pinlineno}%
}%
% prepare reading lines #1 to #2 inclusive
\addtocounter{pinlineno}{-1}%
\let\pin@accu\empty%
\begingroup%
\endlinechar\newlinechar
\@whilenum\value{pinlineno}<#2 \do{%
% use safe catcodes provided by e-TeX's \readline
\readline\pin@file to\pin@line%
\edef\pin@accu{\pin@accu\pin@line}%
\stepcounter{pinlineno}%
}%
\closein\pin@file%
\expandafter\endgroup%
\scantokens\expandafter{\pin@accu}%
}{%
\errmessage{File `#3' doesn't exist!}%
}%
}
\makeatother

==> revision/main_output_logit.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} \\
\hline
Policy tree &      0.0179         &      0.0512\sym{**} &      0.0513\sym{**} &      0.0172         &      0.0528\sym{**} &      0.0527\sym{**} \\
            &    (0.0136)         &    (0.0161)         &    (0.0161)         &    (0.0136)         &    (0.0168)         &    (0.0168)         \\
[1em]
Random      &                     &      0.0323\sym{***}&                     &                     &      0.0338\sym{***}&                     \\
            &                     &   (0.00821)         &                     &                     &   (0.00897)         &                     \\
[1em]
Complexity  &                     &                     &      0.0223\sym{*}  &                     &                     &      0.0242\sym{*}  \\
            &                     &                     &    (0.0104)         &                     &                     &    (0.0113)         \\
[1em]
Requirements&                     &                     &      0.0365\sym{***}&                     &                     &      0.0379\sym{***}\\
            &                     &                     &    (0.0109)         &                     &                     &    (0.0109)         \\
[1em]
Welcome     &                     &                     &      0.0379\sym{***}&                     &                     &      0.0384\sym{***}\\
            &                     &                     &    (0.0107)         &                     &                     &    (0.0107)         \\
\hline
~~Random    &      0.0179         &      0.0190         &                     &      0.0172         &      0.0190         &                     \\
~           &      (.014)         &      (.014)         &                     &      (.014)         &      (.014)         &                     \\
~~Complexity&                     &                     &      0.0290         &                     &                     &      0.0285         \\
~           &                     &                     &      (.015)         &                     &                     &      (.016)         \\
~~Requirements&                     &                     &      0.0148         &                     &                     &      0.0148         \\
~           &                     &                     &      (.015)         &                     &                     &      (.015)         \\
~~Welcome   &                     &                     &      0.0134         &                     &                     &      0.0143         \\
~           &                     &                     &      (.015)         &                     &                     &      (.015)         \\
Estimator   &         OLS         &         OLS         &         OLS         &       Logit         &       Logit         &       Logit         \\
Outcome~mean&         .08         &         .08         &         .08         &         .08         &         .08         &         .08         \\
Observations&        1717         &        6588         &        6588         &        1715         &        6580         &        6580         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}


==> revision/simulation1.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Wed Sep 27 16:37:22 2023
\begin{table}[ht]
\centering
\begin{tabular}{rlrr}
  \hline
 & name & mean & sd \\ 
  \hline
1 & alwaysA & -0.0040 & 0.0784 \\ 
  2 & alwaysB & 0.4965 & 0.0873 \\ 
  3 & alwaysC & 0.2439 & 0.0795 \\ 
  4 & estimated & 0.7085 & 0.0873 \\ 
  5 & known & 0.7073 & 0.0892 \\ 
  6 & random & 0.2459 & 0.0777 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/comparison_table.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Thu Apr 13 04:07:44 2023
names & Always 1 & Always 2 & Always 3 & Random & Policy tree ($d=2$) & Policy tree ($d=3$) & Hybrid tree ($d=2$) & Maximum rule \\ 
  \hline
Nothing &  1.026 &  4.050\starsss &  3.266\starsss &  2.782\starsss &  5.343\starsss &  5.500\starsss &  5.408\starsss &  6.369\starsss \\ 
   & (0.992) & (1.147) & (1.057) & (0.776) & (1.030) & (1.028) & (1.013) & (0.988) \\ 
  Always 1 &      &  3.025\starss &  2.241\stars &  1.756\starss &  4.317\starsss &  4.474\starsss &  4.383\starsss &  5.343\starsss \\ 
   &     & (1.282) & (1.236) & (0.722) & (1.141) & (1.097) & (1.063) & (1.052) \\ 
  Always 2 &      &      & -0.784 & -1.269 &  1.293\stars &  1.449\starss &  1.358\stars &  2.319\starsss \\ 
   &     &     & (1.331) & (0.771) & (0.742) & (0.707) & (0.730) & (0.693) \\ 
  Always 3 &      &      &      & -0.484 &  2.077\starss &  2.234\starss &  2.142\starss &  3.103\starsss \\ 
   &     &     &     & (0.743) & (0.861) & (0.892) & (0.865) & (0.864) \\ 
  Random &      &      &      &      &  2.561\starsss &  2.718\starsss &  2.627\starsss &  3.587\starsss \\ 
   &     &     &     &     & (0.566) & (0.534) & (0.507) & (0.482) \\ 
  Policy tree ($d=2$) &      &      &      &      &      &  0.157 &  0.065 &  1.026\starsss \\ 
   &     &     &     &     &     & (0.293) & (0.315) & (0.297) \\ 
  Policy tree ($d=3$) &      &      &      &      &      &      & -0.091 &  0.869\starsss \\ 
   &     &     &     &     &     &     & (0.251) & (0.240) \\ 
  Hybrid tree ($d=2$) &      &      &      &      &      &      &      &  0.961\starsss \\ 
   &     &     &     &     &     &     &     & (0.227) \\ 
   \hline


==> tables/comparison_table_unknown.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Tue Sep 26 15:40:22 2023
names & Always 1 & Always 2 & Always 3 & Random & Policy tree ($d=2$) & Policy tree ($d=3$) & Hybrid tree ($d=2$) & Maximum rule \\ 
  \hline
Nothing &  1.026 &  4.050\starsss &  3.266\starsss &  2.782\starsss &  5.343\starsss &  5.500\starsss &  5.408\starsss &  6.369\starsss \\ 
   & (0.992) & (1.147) & (1.057) & (0.776) & (1.030) & (1.028) & (1.013) & (0.988) \\ 
  Always 1 &      &  3.025\starss &  2.241\stars &  1.756\starss &  4.317\starsss &  4.474\starsss &  4.383\starsss &  5.343\starsss \\ 
   &     & (1.282) & (1.236) & (0.722) & (1.141) & (1.097) & (1.063) & (1.052) \\ 
  Always 2 &      &      & -0.784 & -1.269 &  1.293\stars &  1.449\starss &  1.358\stars &  2.319\starsss \\ 
   &     &     & (1.331) & (0.771) & (0.742) & (0.707) & (0.730) & (0.693) \\ 
  Always 3 &      &      &      & -0.484 &  2.077\starss &  2.234\starss &  2.142\starss &  3.103\starsss \\ 
   &     &     &     & (0.743) & (0.861) & (0.892) & (0.865) & (0.864) \\ 
  Random &      &      &      &      &  2.561\starsss &  2.718\starsss &  2.627\starsss &  3.587\starsss \\ 
   &     &     &     &     & (0.566) & (0.534) & (0.507) & (0.482) \\ 
  Policy tree ($d=2$) &      &      &      &      &      &  0.157 &  0.065 &  1.026\starsss \\ 
   &     &     &     &     &     & (0.293) & (0.315) & (0.297) \\ 
  Policy tree ($d=3$) &      &      &      &      &      &      & -0.091 &  0.869\starsss \\ 
   &     &     &     &     &     &     & (0.251) & (0.240) \\ 
  Hybrid tree ($d=2$) &      &      &      &      &      &      &      &  0.961\starsss \\ 
   &     &     &     &     &     &     &     & (0.227) \\ 
   \hline


==> tables/descriptives_wave1.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Mon Oct  2 11:36:05 2023
\begin{table}[ht]
\centering
\begin{tabular}{llrrrrr}
  \hline
empty & name & avg & sd & min & max & N \\ 
  \hline
 & Age & 41.79 & 10.95 & 19.00 & 99.00 & 4871 \\ 
   & Female & 0.46 & 0.50 & 0.00 & 1.00 & 4871 \\ 
   & Naturalization application & 0.07 & 0.25 & 0.00 & 1.00 & 4871 \\ 
   & Years in Switzerland & 14.88 & 7.44 & 11.00 & 67.00 & 4871 \\ 
   & Years in Zurich & 9.08 & 4.06 & 3.00 & 20.00 & 4871 \\ 
   & Americas \& Caribbean & 0.05 & 0.22 & 0.00 & 1.00 & 4871 \\ 
   & Asia & 0.06 & 0.25 & 0.00 & 1.00 & 4871 \\ 
   & Central-East Europe & 0.04 & 0.19 & 0.00 & 1.00 & 4871 \\ 
   & Germany and Austria & 0.37 & 0.48 & 0.00 & 1.00 & 4871 \\ 
   & Italy & 0.10 & 0.30 & 0.00 & 1.00 & 4871 \\ 
   & Middle Easy and Northern Africa & 0.01 & 0.12 & 0.00 & 1.00 & 4871 \\ 
   & South-East Europe & 0.12 & 0.32 & 0.00 & 1.00 & 4871 \\ 
   & Spain and Portugal & 0.12 & 0.33 & 0.00 & 1.00 & 4871 \\ 
   & Stateless & 0.00 & 0.04 & 0.00 & 1.00 & 4871 \\ 
   & Sub-Saharian Africa & 0.02 & 0.12 & 0.00 & 1.00 & 4871 \\ 
   & Western Europe & 0.11 & 0.32 & 0.00 & 1.00 & 4871 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/main_output.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{7}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
            &\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}\\
\hline
Policy tree &       1.794         &       5.124\sym{**} &       5.127\sym{**} &       5.004\sym{**} &       5.005\sym{**} &       4.702\sym{**} &       4.758\sym{**} \\
            &     (1.358)         &     (1.609)         &     (1.609)         &     (1.606)         &     (1.606)         &     (1.472)         &     (1.479)         \\
[1em]
Random      &                     &       3.225\sym{***}&                     &       3.245\sym{***}&                     &       3.207\sym{***}&                     \\
            &                     &     (0.821)         &                     &     (0.822)         &                     &     (0.752)         &                     \\
[1em]
Complexity  &                     &                     &       2.230\sym{*}  &                     &       2.260\sym{*}  &                     &       2.199\sym{*}  \\
            &                     &                     &     (1.035)         &                     &     (1.037)         &                     &     (0.938)         \\
[1em]
Requirements&                     &                     &       3.650\sym{***}&                     &       3.711\sym{***}&                     &       3.613\sym{***}\\
            &                     &                     &     (1.095)         &                     &     (1.096)         &                     &     (1.026)         \\
[1em]
Welcome     &                     &                     &       3.787\sym{***}&                     &       3.752\sym{***}&                     &       3.675\sym{***}\\
            &                     &                     &     (1.074)         &                     &     (1.071)         &                     &     (0.986)         \\
\hline
~~Random    &       1.794         &       1.899         &                     &       1.759         &                     &       1.495         &                     \\
~           &     (1.358)         &     (1.361)         &                     &     (1.359)         &                     &     (1.257)         &                     \\
~~Complexity&                     &                     &       2.897         &                     &       2.745         &                     &       2.559         \\
~           &                     &                     &     (1.539)         &                     &     (1.538)         &                     &     (1.432)         \\
~~Requirements&                     &                     &       1.477         &                     &       1.294         &                     &       1.144         \\
~           &                     &                     &     (1.503)         &                     &     (1.499)         &                     &     (1.409)         \\
~~Welcome   &                     &                     &       1.340         &                     &       1.253         &                     &       1.083         \\
~           &                     &                     &     (1.528)         &                     &     (1.527)         &                     &     (1.415)         \\
Estimator   &         OLS         &         OLS         &         OLS         &   PDS lasso         &   PDS lasso         &        DDML         &        DDML         \\
Outcome~mean&        7.69         &        7.92         &        7.92         &        7.92         &        7.92         &        7.92         &        7.92         \\
Observations&        1717         &        6588         &        6588         &        6588         &        6588         &        6588         &        6588         \\
\hline\hline
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}


==> tables/main_output_region5.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{7}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
            &\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}\\
\hline
Policy tree &       1.809         &       5.161\sym{**} &       5.164\sym{**} &       5.013\sym{**} &       5.014\sym{**} &       4.742\sym{**} &       4.782\sym{**} \\
            &     (1.361)         &     (1.608)         &     (1.609)         &     (1.606)         &     (1.606)         &     (1.479)         &     (1.482)         \\
[1em]
Random      &                     &       3.234\sym{***}&                     &       3.253\sym{***}&                     &       3.202\sym{***}&                     \\
            &                     &     (0.820)         &                     &     (0.821)         &                     &     (0.751)         &                     \\
[1em]
Complexity  &                     &                     &       2.243\sym{*}  &                     &       2.268\sym{*}  &                     &       2.199\sym{*}  \\
            &                     &                     &     (1.034)         &                     &     (1.036)         &                     &     (0.938)         \\
[1em]
Requirements&                     &                     &       3.658\sym{***}&                     &       3.725\sym{***}&                     &       3.591\sym{***}\\
            &                     &                     &     (1.094)         &                     &     (1.096)         &                     &     (1.024)         \\
[1em]
Welcome     &                     &                     &       3.793\sym{***}&                     &       3.756\sym{***}&                     &       3.668\sym{***}\\
            &                     &                     &     (1.072)         &                     &     (1.070)         &                     &     (0.984)         \\
\hline
~~Random    &       1.809         &       1.927         &                     &       1.760         &                     &       1.540         &                     \\
~           &     (1.361)         &     (1.362)         &                     &     (1.359)         &                     &     (1.268)         &                     \\
~~Complexity&                     &                     &       2.922         &                     &       2.747         &                     &       2.583         \\
~           &                     &                     &     (1.538)         &                     &     (1.538)         &                     &     (1.433)         \\
~~Requirements&                     &                     &       1.506         &                     &       1.289         &                     &       1.191         \\
~           &                     &                     &     (1.505)         &                     &     (1.499)         &                     &     (1.415)         \\
~~Welcome   &                     &                     &       1.371         &                     &       1.259         &                     &       1.114         \\
~           &                     &                     &     (1.529)         &                     &     (1.527)         &                     &      (1.41)         \\
Estimator   &         OLS         &         OLS         &         OLS         &   PDS lasso         &   PDS lasso         &        DDML         &        DDML         \\
Outcome~mean&        7.69         &        7.92         &        7.92         &        7.92         &        7.92         &        7.92         &        7.92         \\
Observations&        1717         &        6588         &        6588         &        6588         &        6588         &        6588         &        6588         \\
\hline\hline
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}

==> tables/main_output_robustness.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{7}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
            &\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}&\multicolumn{1}{c}{applied}\\
\hline
Policy tree &       2.312         &       5.299\sym{***}&       5.300\sym{***}&       5.194\sym{***}&       5.193\sym{***}&       5.041\sym{***}&       5.012\sym{***}\\
            &     (1.229)         &     (1.437)         &     (1.438)         &     (1.436)         &     (1.437)         &     (1.327)         &     (1.332)         \\
[1em]
Random      &                     &       2.960\sym{***}&                     &       2.989\sym{***}&                     &       2.964\sym{***}&                     \\
            &                     &     (0.729)         &                     &     (0.729)         &                     &     (0.683)         &                     \\
[1em]
Complexity  &                     &                     &       1.760\sym{*}  &                     &       1.807\sym{*}  &                     &       1.770\sym{*}  \\
            &                     &                     &     (0.894)         &                     &     (0.897)         &                     &     (0.834)         \\
[1em]
Requirements&                     &                     &       3.587\sym{***}&                     &       3.656\sym{***}&                     &       3.576\sym{***}\\
            &                     &                     &     (0.990)         &                     &     (0.990)         &                     &     (0.942)         \\
[1em]
Welcome     &                     &                     &       3.521\sym{***}&                     &       3.491\sym{***}&                     &       3.468\sym{***}\\
            &                     &                     &     (0.971)         &                     &     (0.968)         &                     &     (0.908)         \\
\hline
~~Random    &       2.312         &       2.339         &                     &       2.205         &                     &       2.077         &                     \\
~           &     (1.229)         &     (1.231)         &                     &     (1.231)         &                     &     (1.132)         &                     \\
~~Complexity&                     &                     &       3.540         &                     &       3.386         &                     &       3.242         \\
~           &                     &                     &     (1.402)         &                     &     (1.405)         &                     &     (1.296)         \\
~~Requirements&                     &                     &       1.713         &                     &       1.537         &                     &       1.436         \\
~           &                     &                     &     (1.373)         &                     &     (1.371)         &                     &      (1.28)         \\
~~Welcome   &                     &                     &       1.779         &                     &       1.702         &                     &       1.544         \\
~           &                     &                     &     (1.354)         &                     &     (1.356)         &                     &     (1.263)         \\
Estimator   &         OLS         &         OLS         &         OLS         &   PDS lasso         &   PDS lasso         &        DDML         &        DDML         \\
Outcome~mean&        6.17         &        6.48         &        6.48         &        6.48         &        6.48         &        6.48         &        6.48         \\
Observations&        1717         &        6588         &        6588         &        6588         &        6588         &        6588         &        6588         \\
\hline\hline
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
